Prescriptive Process Monitoring for Cost-Aware Cycle Time Reduction

Reducing cycle time is a recurrent concern in the field of business process management. Depending on the process, various interventions may be triggered to reduce the cycle time of a case, for example, using a faster shipping service in an order-to-delivery process or giving a phone call to a customer to obtain missing information rather than waiting passively. Each of these interventions comes with a cost. This paper tackles the problem of determining if and when to trigger a time-reducing intervention in a way that maximizes the total net gain. The paper proposes a prescriptive process monitoring method that uses orthogonal random forest models to estimate the causal effect of triggering a time-reducing intervention for each ongoing case of a process. Based on this causal effect estimate, the method triggers interventions according to a user-defined policy. The method is evaluated on two real-life logs.

==> definitions.tex <==
% Petri Nets
%----------------------------------------------------------
\newcommand{\preset}[1]{^\bullet #1} % PreSet
\newcommand{\postset}[1]{#1^\bullet} % PostSet

\newcommand{\arctgt}[1]{\rightarrow #1}
\newcommand{\larctgt}[2]{\stackrel{#1}{\rightarrow}#2}


==> deleted_text.tex <==
Approach:

% \subsubsection{Discrete Treatment}
% This type of recommendation is useful for situations when a process instance is at risk of running overtime and thus, violating the SLA. In such circumstances, skipping some activities that are optional is a viable choice. But often, skipping an activity, although optional, can result in some costs, such as a decrease in quality. Therefore, it is helpful to know how much skipping an activity has an effect on the overall cycle time. Furthermore, in situations when the process owner is not willing to skip all optional activities, this recommendation can be used to choose which of the optional activities is the best to skip for a particular case.

% This type of treatment is for situations where the treatment either happens or it does not. It is used in situations when a possible treatment is identified, but the cost of applying that treatment to every case is too high. So, the analyst would like to know which cases should receive that treatment. Also, this treatment type is used when there are several treatment options available and we would like to know which case should receive which treatment. For each possible treatment, we construct an ORF model and we use it to obtain a treatment effect for an input prefix. For each ORF, a boolean treatment indicator $T$ is supplied in addition to the $X$ and $W$. This treatment indicator is equal to $1$ if the treatment was applied in that trace and $0$ otherwise. After the ORF models are constructed for each possible treatment, running cases are transformed into feature vectors by the same encoding method as in the offline phase. They are then supplied to the trained model, which outputs a treatment effect for each running case. 

% Since the goal is to minimise the target variable which is case duration, the treatment that has a higher treatment effect value is selected is considered the most problematic for that particular running case. So in cases where the goal is to choose an activity to skip, the one with the highest treatment effect is picked. If there is only one optional activity, then that activity can be skipped if their treatment effect is higher than a threshold, previously determined by the user.

% \subsubsection{Continuous Treatment}
% The same procedure as the discrete treatment type is used when the treatment is a continuous value. However, the way the estimated effect is interpreted is different in continuous treatments. If the treatment is binary, the treatment effect is difference in potential outcomes  $Y^{t=1}$ and $Y^{t=0}$. However, this interpretation cannot be used when the treatment is not binary. Hence in continuous ORFs, since the relationship between $T$ and $Y$ considered to be linear, the resulting treatment effect is the slope of this linear model.

% For example, if treatment effect $\tau$ is estimated to be $3$ for a case, it means that if the treatment value for that case was set to $T=m$, then that would cause the outcome to become $Y=3m$.  
% In some situation where the process workers have the option to perform an activity at different times, our recommendation system can provide insight into when is the best time for that activity to be executed. In such cases, we build a continuous ORF with the treatment indicator being the time (in days) since start of the case when that activity occurred.

% at decision time, all the ongoing cases that are at a stage in the process where a decision regarding their treatment should be made are encoded into feature vector using the same encoding approach as the offline phase. Then, using the pre-trained ORF at the offline phase, a treatment effect is estimated for each of them. Finally, these cases are ranked according to their treatment effects and based on the previously selected policy, top $n$ percent of them are selected to be treated.


% The final step of this method after all ORFs are constructed and the treatment effects and confidence intervals are estimated is to rank the recommendations. We propose a two dimensional ranking approach. One dimension is the net benefit of applying the treatment. The other dimension is the confidence of each estimated treatment effect. Then ranking are visualised via a modified version of PICK charts, which are commonly used in the field of process improvement. The y-axis in the PICK chart is the net benefit of applying the treatment. We calculate the net benefit similar to \cite{} and use the following notation:
% \begin{itemize}
%     \item $v$: value (benefit) of the reduction in cycle time, assuming that it is constant and given as prior knowledge; 
%     \item $p$: the probability of that specific case violating the SLA
%     \item $c$: impression cost for a treatment; 
%     \item $u$: the treatment effect; and
% \end{itemize}

% We define the net benefit of applying the treatment is as follows:

% \begin{center}
%     $net = p \times (u \times v - c)$.
% \end{center}

% The x-axis in the PICK chart is the confidence of each estimated treatment effect. The confidence is calculated by taking the inverse of the difference between the upper bound of the confidence interval $U$ and the lower bound $L$.
% \begin{center}
%     $Confidence = 1 / (U - L)$.
% \end{center}

% Similar to regular PICK charts, we have four quadrants, which are named in a slightly different way. The quadrants in the chart are defined as follows: 

% \begin{itemize}
%     \item \emph{Possible}: low payoff, high confidence
%     \item \emph{Implement}: high payoff, high confidence
%     \item \emph{Investigate}: high payoff, low confidence 
%     \item \emph{Kill}: low payoff, low confidence
% \end{itemize}

% \noindent The cases that fall into the quadrant \emph{possible}, have low payoff, but the confidence in the treatment effect makes them possible candidates to receive the treatment. The Implement quadrant describes cases where the payoff is high, meaning that the process instance is in high risk of violating the SLA, the benefit of reducing that case's cycle time is high and the treatment effect is estimated to be high. In addition, these cases have treatment effects that have a high confidence. Therefore the are the priority cases that should receive the treatment. The investigate quadrant refers to cases that benefit from receiving the treatment, however, the estimate treatment effect for these cases do not have high confidence. In these cases a domain expert should investigate further if this case indeed benefits from receiving the treatment. Lastly, the \emph{kill} quadrant contains cases that do not benefit from the treatment and the estimated treatment effect for them is not confident. Therefore, there is no need for these cases to be treated.



% % \begin{itemize}
% % \vspace{-6pt}
% %     \item Highly confident
% %     \item Somewhat confident
% %     \item Not confident
% % \end{itemize}

% These groups are determined based on the length of the confidence intervals and the input from the user. For example, if the user indicates that they require a $d1$ number of days confidence, but a $d2$ number of days interval is also acceptable (note that $d1<d2$), the recommendations will be ranked the following way: The cases where the length of the confidence interval is $d1$ days or less will be regarded as highly confident. If the length of the confidence interval falls between $d1$ and $d2$ then those cases are classified as somewhat confident. And finally, if the length of the interval is above $d2$, those results are not confident. It should be noted that the choice of $d1$ and $d2$ is decided by a domain expert and should be based on a cost model that includes the likelihood of the cases running overtime, the cost of running overtime and the cost of the treatment.

% Based on this ranking strategy, we use the following policy for following the recommendations: \emph{Highly confident} are safe enough to follow without major human examination. Therefore, if they recommend that the treatment should be applied, then it is safe to do so. In cases where the results are \emph{somewhat confident}, the recommendations should only be followed if a domain expert can validate those results. The remaining \emph{not confident} results are discarded and the decision on whether to apply the treatment on those cases should be purely based on the opinion of the domain expert.  

% The first group \emph{highly confident} refers to cases where the higher and lower bound of the confidence intervals are not close to $0$ and also the confidence interval does not include $0$. For example, if the estimated treatment effect is $8$ and confidence interval is [5,10]. This range tells us that the treatment has an effect between $5$ and $10$. So, in the even in the worst case we observe a treatment effect of $5$. So the ORF is confident that there is a positive treatment effect in this case. In the second group \emph{somewhat confident}, one of the bounds of the confidence interval falls close to $0$. For example, consider a case where the estimated treatment effect is $5$ but the lower bound of the confidence interval is $0.5$. This indicates that due to sampling variability, the ORF is not completely sure if there is a significant effect on the target variable. So, extra caution should be taken with dealing with cases that fall within this group. The third group \emph{Not confident} refers to case where the confidence interval includes $0$. An example of this is case where the confidence interval is [-5,5]. Such an interval shows that the algorithm is undecided whether the treatment has a positive effect or negative. Therefore, these results should be discarded.

Evaluation:

% \subsubsection{BPI17:} This log shows a number of cases with unusually long duration, which severely impacts customer experience. However, since this is an interactive process, meaning that there may be one or more interactions with the customers, simply deciding to skip an activity may not always lead to a decrease in duration. This is because in some instances, the long duration is due to the fact that the company is waiting for some input in the customer. To deal with the problem of long duration, the authors of \cite{} recommend the bank to be constantly in contact with the customer. They argue that frequent contact with the customer will result in them providing the required input or answers more quickly, thus resulting in a shorter cycle time. While this is true for many of the cases observed in this log, the cost of calling each and every customer might be too high for this recommendation to be effective. So, with our recommendation system based on orthogonal random forests, we address this issue. We constructed two ORFs. One with the treatment options being whether to perform the activity \emph{W\_Call incomplete files}, another performing or skipping \emph{W\_Assess potential fraud}. We then proceed to estimate treatment effects and 90\% bootstrap confidence intervals for each trace prefix in the test set. We then apply the ranking criteria to our recommendations. We discard the results with poor confidence and only keep those which are ranked as 'strongly recommended' and 'treat with caution'. As expected, for both treatments, a variety of treatment effects are estimated, suggesting that a blanket treatment for all cases is not optimal. For example, in one case the treatment effect for activity W\_Assess potential fraud is 2 days but for activity W\_Call incomplete files the effect is estimated to be 9 days. After having a closer look at the input prefix of this trace, we realised that it has a similar structure to cases where the activity W\_Call incomplete files takes a long time to finish. This suggest that our method can identify cases where the customer is not responsive, therefore it would be beneficial for the company to proceed without asking this customer for additional documents. In another example, we observe a high treatment effect of skipping W\_Assess potential fraud for a case. We observe that this is a low credit customer applying for a large loan, which is likely to to go through fraud assessment. So, we can conclude that skipping this activity is a better option, and instead, the bank can request further information about the customer earlier in the process to avoid the lengthy fraud assessment procedure.

% In another recommendation in the BPI challenge 2017 report \cite{}, the authors recommend to send offers as early as possible, because they observe a correlation between sending offers early and customers being more responsive, and therefore, having shorter cycle times. This recommendation, however, may not always be possible to follow. The company has limited resources and it is not always practical to send offers early for each case. So, we construct an ORF with the treatment being the time since the start of the case when the first offer was sent to the customer. This is an example of a continuous treatment. Our results show that sending offers early does indeed have an effect of the reduction of cycle time, with the median treatment effect being 1.2 days, which is in accordance with the findings of the winning report of the challenge. However, we again see great variability in effects in different cases. So, these treatment effects can be used to prioritise the cases where sending offers early positively affects customer responsiveness and in turn, reduces cycle time.

% \subsubsection{BPI19:} In this dataset, we observe several types of change to purchase order items. Since, changes might lead to re-work, we hypothesise that avoiding these changes leads to lower cycle times. This is one of the recommendations of one of the participants of the challenge \cite{}. They used a random forest to predict cycle time. They did it repeatedly each time including additional variables to identify problematic activities that affect cycle time. They made the conclusion that change activities have higher impact on cycle time and recommended to thoroughly check the initial order for correctness of price, quantity, and justifiability for order placement. However, fixing price, quantity and approval of POs all at the same time for each case without taking into account the specific context of each case leads to a rigid order placement procedure. Our method calculates treatment effects and confidence intervals of each type of change and for each case we can determine which type of change has a higher effect on duration. In this way, we can avoid the most problematic activity while at the same time, preserve the flexibility required for each process instance. For example, in a case where the treatment effect of changing the price is higher than the treatment effect of changing quantity, the user can perform initial checks for the price or fix the price without the possibility of change, but retain flexibility over quantity, in case it is revealed the a different number of the goods is required. Also, we observe treatment effects are close to zero for some cases. This indicates that for a case with those specific features, making changes does not affect the outcome. Recommendations based on traditional machine learning methods such as random forests used in \cite{}, are not personalised. Therefore, these recommendations are applied even to cases where the recommendation does not have an effect on the target, whereas in our method we can identify cases where the treatment is actually required. In many causal machine learning methods, including ORFs, used in this approach, effects of interventions are considered to be heterogeneous and so, in this regard, they outperform traditional machine learning methods. 
